Materials Matter: Investigating Functional Advantages of Bio-Inspired Materials via Simulated Robotic Hopping

In contrast with the diversity of materials found in nature, most robots are designed with some combination of aluminum, stainless steel, and 3D-printed filament. Additionally, robotic systems are typically assumed to follow basic rigid-body dynamics. However, several examples in nature illustrate how changes in physical material properties yield functional advantages. In this paper, we explore how physical materials (non-rigid bodies) affect the functional performance of a hopping robot. In doing so, we address the practical question of how to model and simulate material properties. Through these simulations we demonstrate that material gradients in the leg of a single-limb hopper provide functional advantages compared to homogeneous designs. For example, when considering incline ramp hopping, a material gradient with increasing density provides a 35% reduction in tracking error and a 23% reduction in power consumption compared to homogeneous stainless steel. By providing bio-inspiration to the rigid limbs in a robotic system, we seek to show that future fabrication of robots should look to leverage the material anisotropies of moduli and density found in nature. This would allow for reduced vibrations in the system and would provide offsets of joint torques and vibrations while protecting their structural integrity against reduced fatigue and wear. This simulation system could inspire future intelligent material gradients of custom-fabricated robotic locomotive devices.

==> Archive/09152024_discussion.tex <==
The results of these experiments, and how they compare to the prior experimental results with isotropic materials, are illustrated in \fig{fig:5}. Remarkably, the results with the anisotropic materials still yield significant functional advantages for tracking error, but with a reduced power consumption compared to isotropic materials. Additionally, it is interesting to note that the order of the functional gradients does appear to influence the performance. Specifically, the fact that $\rho$-inc and $\rho$-dec are different implies that materials are interacting with each other, not simply combining into one bulk \textit{equivalent} material. 

% Proceeding beyond the tunability of density and porosity shifts impacting functional features of the materials, we look at now varying the three springs in the hopper link. The actual material of the ankle joint contacts with a softer material of the foot pad and shifts to a stiff bone before shifting again to the soft tendon-muscle connection. 

% In viewing the density functional gradient, we find that we minimize the tracking error with a functionally graded density increase and decrease. However, the power increases significantly for a normalized hop height of 1m. In looking at the impact of shifting the material functional gradient, we find that material gradients, both increasing and decreasing, allow nonsignificant changes in power while significantly reducing tracking error and reducing the amount of jerk experienced in the joint. 

% Specifically, increasing the material from the joint to the foot provides a significant benefit, minimizing jerk while avoiding the functional disadvantages of stainless steel's heaviness. 

\section{Conclusions and Future Work}
\label{sec: conclusions}
In this paper, we utilize simulation as a method for evaluating how material properties and bio-inspired relationships impact robotic behaviors across various locomotive tasks. Our results find that material properties significantly influence robotic performance, with isotropic materials yielding functional trade-offs. 
% These trade-offs can be tuned to maximize specific robotic behaviors by purpose-built biological inspiration, as done in \cite{schulz_conservation_2023,berger2018conservation}.
Our results also determine that material anisotropies provide several functional advantages over isotropic designs. Specifically, materials with increasing density gradients yield reduced tracking error, reduced power consumption, and reduced jerk compared to mono-materials. These functional gradients, while abundant in nature (for example in plant roots, human skin, animal whiskers, and the Achilles tendon), are rarely utilized in mechanical design. We hope that our results inspire future designs that leverage these functional benefits. 

Notable limitations of our methodology include the slow simulation speeds required to model porous and/or stiff materials. This limitation is exacerbated by the fact that very few simulation tools currently model physical material properties in computationally tractable ways. By demonstrating the importance of material selection on robotic performance, we hope that the results will motivate future work towards efficiently modeling physical materials for robotic systems. 
An additional limitation of our work is that we do not account for material failure or fatigue. Thus, future work is needed to evaluate the durability of these materials under cyclic testing. 
% Explicitly, we characterize the metal-ceramic group as belonging to the range:
% \begin{align*}
%     \rho_{m,c} &\in [1.75 \times 10^{3}\ , 2.25 \times 10^{4}]\ \text{kg/m}^3, \\
%     \text{E}_{m,c} &\in [1.1\times 10^1\ , 1\times 10^3]\ \text{GPa},
% \end{align*}
% and the polymer-natural composites group as belonging to the range: 
% \begin{align*}
%     \rho_{p,nc} &\in [5\times 10^{2}\ , 3.5\times 10^3]\ \text{kg/m}^3, \\
%     \text{E}_{p,nc} &\in [1\times 10^{-1}\ , 9 \times 10^0]\ \text{GPa}.
% \end{align*}
The key takeaway of this work is that the inherent complexities of materials drive functional improvements in robotic systems. This motivates further study, particularly of anisotropic materials, to understand how physical properties influence performance. It also highlights the importance of advancing research and developing simulation tools to model these complexities for real-world applications.
% This underscores the need for continued research into the role of materials in robotic systems and the development of simulation tools to model these complexities for real-world applications.

% for modeling the complexities of physical materials in ways that are practical enough to be used towards robotic simulation. 

% These functional advantages are es propose that more advanced robotic locomotion modes could indicate further benefits from the anisotropy of biological composites. 


% these functional changes can be optimized through purpose-built hardware customized to a specific application. 


% However, adding material properties like porosity and stiffness can alter key performance indicators of robotic locomotion during different behaviors. 


% A framework for finding the purpose-built material relationship in these robotic systems is to inspire the material relationship from the functional gradients 

% In this paper, we showed that materials can have large functional benefits and trade-offs, and these trade-offs can be tuned to maximize specific robotic behaviors by purpose-built biological inspiration. Future robotic systems could implement and inspire their mechanical segments to allow for similar functional benefits. 

% Traditionally, robotic material design is very opportunistic, utilizing sensors, actuators, and linkages taken from other fields and then opportunistically applied to robotics. A prime example includes camera-based tactile sensors on grippers that utilize off-the-shelf cameras but often modify the rest of the hardware~\cite{andrussow_minsight_2023,do_densetact_2023}. In this paper, we show that simulation can be a cost-efficient way to determine an optimized material set and arrangement for purpose-built tasks.

% In some fields of hardware development, like conservation technology, engineers have begun to adopt purpose-built hardware customized to the specific application as it increases efficacy~\cite{schulz_conservation_2023,berger2018conservation}. Robotic tasks are often bio-inspired by the biomechanics of reaching or walking of humans~\cite{ames_human-inspired_2014} or other wildlife~\cite{burden_why_2024,badri-sprowitz_birdbot_2022,patel_rapid_2014}. 


% As there are limitations to what is possible in common robotic simulation platforms like MuJoCo, perfectly recreating the material mechanics is impossible given the current programming. In this paper, we show the ability of porosity and stiffness shifting to drive mechanical functional differences. However, this work does not look at material failure or fatigue. Future work would need to look into the ability of these materials to not degrade from cyclic testing. 
